Optimal periodic structures with general space group symmetries in the Ohta-Kawasaki problem

We consider the problem of rigorously computing periodic minimizers to the Ohta-Kawasaki energy. We develop a method to prove existence of solutions and determine rigorous bounds on the distance between our numerical approximations and the true infinite dimensional solution and also on the energy. We use a method with prescribed symmetries to explore the phase space, computing candidate minimizers both with and without experimentally observed symmetries. We find qualitative differences between the phase diagram of the Ohta-Kawasaki energy and self consistent field theory when well away form the weak segregation limit.

==> notation.tex <==
%!TEX root = ms.tex

\red{Check all appearances of $\|\cdot\|_{\sym}$}

Since are interested in periodic critical points of $\EEE$, we expand $u$ as  
\begin{equation}\label{e:Fourier}
  u (\x)= \sum_{k \in \Z^3} c_k \exp(\textup{i} \L k \cdot \x),
\end{equation}
for some invertible $3 \times 3$ matrix $\L$.
\red{This is not the same $L$ as in the code!}
The Laplacian corresponds to a diagonal operator on the Fourier coefficients
\[ 
  -\Delta u (\x) = 
  \sum_{k \in \Z^3} \DLk c_k \exp(\textup{i} \L k \cdot \x)
\]
where
\[
  \DLk \bydef \sum_{j=1}^{3} ( \L k )_j^2 .
\]

\begin{remark}
To relate $\L$ to periodicity in $\x$ we observe that $u(\x+2\pi (\L^{-1})^T \vec{e}_j) = u(\x)$ for $j=1,\dots, 3$, where $\{\vec{e}_j\}_{j=1}^3$ form the standard basis of $\R^3$. In particular, $\Omega$ is the parallelepiped given by $ \{\x \in \R^3 : \x =  2 \pi (\L^{-1})^T \tilde{\x} \text{ with } \tilde{\x} \in [0,1]^3 \}$.
\end{remark}

\begin{remark}
To optimize over the length scale(s) we will need to be able to scale the vectors in the unit cell. We incorporate this into $\L$ by decomposing it as
\[
  \L = \ls \left( \begin{array}{ccc} 
  \ell_1 & 0 & 0 \\
  0 &  \ell_2 & 0 \\
  0 & 0 & \ell_3 
  \end{array} \right).
\]
This thus corresponds to the fundamental domain
\[
  \{\x \in \R^3 : \x =  2 \pi (\ls^{-1})^T \hat{\x} \text{ with } \hat{\x} \in [0,1/\ell_1] \times [0,1/\ell_2] \times [0,1/\ell_3] \} .
\]
\end{remark}


In addition to periodicity we assume
 invariance under some space group $\G$:
\[
  u(C_g \x + 2\pi  (\L^{-1})^T  D_g)=u(\x) \qquad\text{for all } g \in \G,
\]
where $C_g$ is an orthogonal matrix ($C_g^{-1} = C_g^T$), and $D_g \in [0,1]^3$.
We will consider space groups $\geq 16$ \red{but may still have to exclude ones that allow for a continuous shift, which you can see from the Coxeter notation by the fact that there is only one number between the brackets (I don't know why).} The groups we deal with in this paper are
16--24, 47--74, 81--98, 111-142, 147-155, 162--167, 174--182, 187-230.

Several remarks are in order to describe the relation between symmetries, encoded in the space group, and periodicity.

\begin{remark}\label{r:match}
The symmetries may imply that some of the length scales are not independent. 
In particular, depending on the type of group $\G$, there are one, two or three independent scale variables $\ls_j$. 
We denote the number of independent length scales by $J$.
For the orthorhombic groups (\red{which numbers?}) we have $J=3$ and we simply set  $\ell_j = \ls_j$ for $j=1,2,3$.
For the tetragonal (\red{which numbers?}), trigonal (\red{which numbers?}) and hexagonal (\red{which numbers?}) groups we have $J=2$: $\ell_1=\ell_2=\ls_1$
and $\ell_3 = \ls_2$. For the cubic groups (\red{which numbers?}) we have $J=1$,
hence $\ell_1=\ell_2=\ell_3 =\ls_1$. 
In particular, we introduce the dilation matrices $\hLLl$ as follows:
\[
  J=3:~ \hLLl  \bydef 
  \left( \begin{smallmatrix}
    l_1 & 0 & 0 \\
    0 &  l_2 & 0 \\
    0 & 0 & l_3 
    \end{smallmatrix} \right) ,
	\qquad
  J=2:~ \hLLl \bydef   
  \left( \begin{smallmatrix}
    l_1 & 0 & 0 \\
    0 &  l_1 & 0 \\
    0 & 0 & l_2 
    \end{smallmatrix} \right),
	\qquad
  J=1:~ \hLLl \bydef   
  \left( \begin{smallmatrix}
    l_1 & 0 & 0 \\
    0 &  l_1 & 0 \\
    0 & 0 & l_1 
    \end{smallmatrix} \right) .
\]

The coordinates are thus group according to which independent length scale they are linked.
The matrices $C_g$ act block-wise 
on these grouped coordinates in the sense that
$C_g$ is diagonal when $J=1$, while when $J=2$ then $C_g$ is blockdiagonal with blocks of size $2$ and $1$: $(C_g)_{ii'}=0$ for $i=1,2$, $i'=3$ and for 
$i=3$, $i'=1,2$. We say that $C_g$ has a periodicity compatible block structure.
A different way to characterize this compatibility is through the commutative property
\[
    C_g \hLLl = \hLLl C_g \qquad \text{for any } l \in \RJ_+ \text{ and any } g\in \G.
\]
\end{remark}

\begin{remark}
For the orthorhombic, tetragonal and cubic space groups we choose $\ls$ to simply be the identity. For the tetragonal and trigonal space groups we choose
\[
  \ls = \ls_{\triangle} \bydef \left( \begin{array}{ccc}
  \sqrt{3}/2 & 0 & 0 \\
  -1/2 & 1 & 0 \\
  0 & 0 & 1
   \end{array} \right) .
\]
\red{This is not yet used in the code, but I think it is ``better''.}
\red{Need to check that this matches the way the symmetries have been implemented.}
We note that $\ls_{\triangle}$ communtes with $\hLLl$ for $J=2$ and any $l\in \R^2_+$. 
\end{remark}

The compatibility between the independent length scales and symmetry group
decribed in Remark~\ref{r:match} implies that
we may simplify the description of $\DLk$ as follows.
No cross product terms $\ls_j \ls_{j'}$ with $j \neq j'$ appear in the expression for $\DLk$. This motivates us to
introduce $\kappa_j=\ls_j^2$.
We distinguish four cases and in each write 
$\DLk=\Dkk$, where,  
depending on the type of space group,
\begin{alignat*}{3}
\text{orthorhombic}:&\quad&
\Dkk &\bydef \kappa_1 k_1^2  + \kappa_2 k_2^2 + \kappa_3 k_3^2 && J=3,\\
\text{tetragonal}:&& 
\Dkk &\bydef \kappa_1 (k_1^2 + k_2^2) + \kappa_2 k_3^2  && J=2,\\
\text{trigonal and hexagonal}:&&
\Dkk &\bydef \kappa_1 ( k_1^2 - k_1 k_2  + k_2^2 )  + \kappa_2 k_3^2 && J=2, \\
\text{cubic}:&&
\Dkk &\bydef \kappa_1 (k_1^2 + k_2^2 + k_3^2) &\qquad& J=1. 
\end{alignat*}
We summarize these as 
\[
  \Dkk = \sum_{j=1}^J \Dkj{j} \kappa_j,
 \qquad\text{where } \Dkj{j} \in [0,\infty) 
 \text{ for all }k\in \Z^3 \text{ and } 1\leq j \leq J.
\]
Clearly $\Dkk$ is linear in $\kappa$ for fixed $k$, while it is a positive
definite quadratic form in $k$ for fixed $\kappa \in \RJ_+$. The
linearity in $\kappa$ will be most important, hence it is stressed by choosing
the notation~$\Dkk$. On occasion we will also interpret, for fixed $k$, \
the vector
$\Dk = \{\Dkj{j}\}_{j=1}^J$ as an element of the dual of $\RJ$.

To recover $\L$ from $\kappa$ we use $\L = \L_\kappa \bydef \ls \hLLl[\sqrt{\kappa}]$.
The corresponding domain of periodicity is denoted by
\begin{equation}\label{e:omegakappa}
  \Omega_\kappa \bydef 
  \{\x \in \R^3 : \x =  2 \pi (\L_\kappa^{-1})^T \tilde{\x} 
                       \text{ with } \tilde{\x} \in [0,1]^3 \} .
\end{equation}

\begin{remark}\label{r:Cgmapslattice}
The matrices $C_g$ for $g \in \G$ respect the periodicity symmetry in the sense that $C_g$ (as well as $C_g^T$) maps the lattice $\ls \Z^3$ to itself.
Since $C_g$ is orthogonal 
 and is periodicity symmetry compatiblein the sense explained in Remark~\ref{r:match},
$C_g$ also maps the lattice 
$\L_\kappa \Z^3$ to itself for any $\kappa \in \R^J_+$ and $g \in \G$. Moreover, we have 
\begin{equation}\label{e:DkjCginvariance}
  \Dkj[\ls^{-1} C_g \ls k]{j} =\Dkj[k]{j} \qquad\text{for any }
  k\in \Z^3, 1\leq j \leq J, \text{ and } g \in \G.
\end{equation}
\end{remark}

We aim to find stationary points (e.g.\ minimizers \red{remark in intro on this}) of the energy $\EEE$ with respect to variations in the Fourier coefficients $c_k$, under the constraint $c_0=m$, and length scales $\kappa \in \RJ_+$:
\begin{equation}\label{e:defE}
  E(\kappa,c) \bydef 
      \frac{1}{2} \sum_{k \in \Z^3 \setminus \{0\}} \PP(\Dkk) \, c_k c_{-k}
  \, +  \frac{1}{4} \conv{c^4}_0  -\frac{m^4}{4} .
\end{equation}
Here $\PP:(0,\infty) \to \R$ is given by
\[
  \PP(y) \bydef \frac{1}{\gamma^2} \,\! y  - 1 + \frac{1}{y} .
\]
We will use that for large Fourier modes $\PP(\Dkk)$ has fixed sign (positive) and its size increases monotonically. Indeed 
\begin{alignat}{2}
 |\PP(y)| & > 0  &\qquad&\text{for all } y > \yP, \label{e:PyP1} \\
 \frac{\PP'(y)}{P(y)} & > 0 &\qquad&\text{for all } y > \yP, \label{e:PyP2}
\end{alignat}
where 
\begin{equation}\label{e:defy0}
  \yP \bydef \begin{cases}
   \gamma  & \quad\text{for } \gamma \leq 2,\\
   \frac{2\gamma}{\gamma-\sqrt{\gamma^2-4}}
    & \quad\text{for } \gamma > 2.\\
   \end{cases}
\end{equation}
The parameter range $\gamma \leq 2$ is included for completeness only. No pattern formation is observed in that regime due to global convexity of the energy functional~\cite{someChoksipapers}.

Throughout this paper we use the notation $\conv{c \, c'}$ for the discrete convolution product
\[
\conv{c \, c'}_k \bydef \sum_{k_1+k_2=k} c_{k_1} c'_{k_2},
\]
which naturally extends to powers. In particular
 \[
   \conv{c^4}_0 = \sum_{k_1+k_2+k_3+k_4=0} c_{k_1} c_{k_2} c_{k_3} c_{k_4} .
 \] 
The normalization of $E$ is such that the trivial uniform state has zero energy.

In Fourier space the PDE~\eqref{e:PDEOK} is transformed to
\begin{equation}\label{e:fk}
  f_k(\kappa,c) \bydef  \PP(\Dkk) c_k + \conv{c^3}_k  =0
\end{equation}
for $k \in \Z \setminus \{0\}$.
\begin{remark}\label{r:dEdc}
Indeed, by using that $\Dk[-k] = \Dk$ we see that $\frac{\partial E}{\partial c_{k}}=f_{-k}$ for all $k \in \Z \setminus \{0\}$.
\end{remark}
Stationarity of the energy with respect to variations in $\kappa$
is equivalent to 
\begin{equation}\label{e:hj}
  h_j(\kappa,c) \bydef \frac{1}{2} \sum_{k \in \Z^3 \setminus \{0\} } \PP'(\Dkk)  \, \Dk^j \, c_k c_{-k} = 0,
\end{equation}
for $1 \leq j \leq J$.
Namely,
\begin{equation}\label{e:dEdkappa}
    \frac{\partial E}{\partial \kappa_j}(\kappa,c)= h_j(\kappa,c)  =0
	\qquad \text{ for all } j =1,\dots,J,
\end{equation}
corresponds to stationarity of the energy $\EEE$ with respect to variations in the proportions of the fundamental domain of the periodicity cell $\Omega$ which respect the symmetry type (in the sense of Remark~\ref{r:match}).

\begin{remark}
We will not describe one- and two-dimensional cases separately, but they are coded up \red{Needs to be done of course}
\end{remark}

For $u$ a real-valued function, we have the symmetry $c_{-k}=c_k^*$, and in particular $c_k c_{-k} = |c_k|^2$. However, we choose to work over $\C$ throughout without requiring $c_{-k}=c_k^*$, 
as this unifies some of the arguments. 
In Definition~\ref{def:conjugation} we will introduce a conjugation operator which is exploited to recover real-valuedness of the solution, see Theorem~\ref{thm:contraction}.

We choose as the norm on the Fourier indices
\begin{equation}\label{e:knorm}
   \knorm \bydef \sqrt{\Dk \bkappa},
\end{equation}
for some $\bkappa \in \R^J_+$ to be fixed later.
Indeed, $\bkappa$ will be chosen to be the numerical approximation of the optimal domain size parameters. 
On the set of Fourier coefficients we introduce the norm on 
\begin{equation}\label{e:nu-norm}
  \| c \|_\nu   \bydef  \sum_{k \in \Z^3} |c_k|  \nu^{\knorm}.
\end{equation}

On $\RJ$ and $\CJ$ we  choose the norm
\begin{equation}\label{e:normFJ}
   | \kappa |_{\FFJ} \bydef \max_{j=1,\dots,J} \frac{|\kappa_j|}{\bkappa_j} 
  \qquad \text{for } \F = \R \text{ and } \F=\C.
\end{equation}
The norm on the dual is then given by 
\[ 
  | q |^*_{\FFJ}  \bydef \sum_{j=1}^J |q_j|  \bkappa_j 
  \qquad\text{for } q = \FFJ.
\]
In particular, this choice of norm has the convenient property 
(writing $\Dk = (\Dkj{j})_{1\leq j\leq J}$)
\begin{equation}\label{e:choice}
  | \Dk |^*_{\FFJ} = \Dk \bkappa, 
   \qquad \text{for } \F = \R \text{ and } \F=\C.
\end{equation}

\begin{definition}\label{def:conjugation}
On $\CJ$, $\C^{\Z^3}$ and then on $\CJ\times \C^{\Z^3}$ we introduce the conjugation operation
\begin{alignat*}{1}
  (\gammaconj \kappa)_j &\bydef \kappa_j^* \\
  (\gammaconj c)_k & \bydef c^*_{-k} \\
  \gammaconj (\kappa,c) & \bydef (\gammaconj \kappa, \gammaconj c).
\end{alignat*}
\end{definition}
The convolution product is $\gammaconj$-equivariant:
\[
  \conv{\gammaconj c \, \gammaconj c'} = \gammaconj \conv{c \, c'}.
\]
It then follows from the formulas~\eqref{e:fk} and~\eqref{e:hj} for $f$ and $h$,
combined with the fact that $P$ is real analytic, that
\begin{equation}\label{e:hfconjequivariant}
  \gammaconj \bigl(h(\kappa,c),f(\kappa,c) \bigr) =
  \bigl(h(\gammaconj(\kappa,c)),f(\gammaconj(\kappa,c)) \bigr),
\end{equation}
and intimately related to this (since $f$ and $h$ correspond to the partial derivatives of $E$)
\[
  E(\gammaconj(k,c)) = E(k,c)^*.
\] 


==> setup.tex <==
%!TEX root = ms.tex

We write $\FJ_+ = \{ \kappa \in \FJ : \re \kappa_j >0 \}$
and define $\FF : \FJ_+ \times \X_0 \to \FJ \times \tX_0$ by
\begin{equation}\label{e:defFF}
\FF (\kappa,b) \bydef \bigl[H(\kappa,b),F(\kappa,b) \bigr] \bydef \bigl[ 
(h_j(\kappa,\sigma(m\e_0+b)))_{j=1,\dots,J} , 
(f_k(\kappa,\sigma(m\e_0+b)))_{k \in \X_0} \bigr].
\end{equation}
Here the Fourier part of the codomain can be chosen to be
\[
  \tX_0 \bydef \Bigl\{ (b_k)_{k \in \ZY_0} : \textstyle\sum_{k \in \ZY_0} \min\{1,|P(\Dk 1)|\} \, |b_k| \, \omega_k < \infty \Bigr\}.
\]
Projections onto $\FJ$ is denoted by $\pi_\kappa$,
whereas the projections on $\X_0$ and $\tX_0$ are both denoted by~$\pi_b$. 

We can use Lemma~\ref{l:symquad} to rewrite $H$ as
\begin{alignat}{1}
	H_j(\kappa,b) & = 
	\frac{1}{2} \sum_{k \in \Z^3 \setminus \{0\} } \PP'(\Dkk)  \, \Dk^j \, (\sigma(m\e_0+b))_k (\sigma(m\e_0+b))_{-k} \nonumber \\
    & = 
   	\frac{1}{2} \sum_{k \in \ZY_0 }  \PP'(\Dkk)  \, \Dk^j \, |\Gacts| \, b_k 
	(\sigma(m\e_0+b))_{-k}  \label{e:Hrewrite}.
\end{alignat}
Furthermore, $F$ naturally splits into a linear (in $b$) and nonlinear part:
\[
  F_k(\kappa,b) = P(\Dk \kappa ) b_k + \Phi_k(b), \qquad \text{for any } k \in \ZY_0,
\]
where
\begin{equation}\label{e:defPhi}
  \Phi(b) \bydef  \conv{(\sigma(m\e_0+b))^3}.
\end{equation}

To perform numerical computations, and to set up a Newton-like fixed point scheme, we perform a finite dimensional projection
For $K >0$ we define the finite cut-off index sets 
\begin{alignat*}{1}
  \Z^K & \bydef \{ k \in Z^3 : \kk \leq K \},  \\
  \Z^K_0 & \bydef \Z_0 \cap \Z^K.
\end{alignat*}
We denote by $N$ the number of elements in $\Z^K_0$.
We set
\[
  \XK = \{ b \in \X_0 : b_k =0 \text{ for all } k \notin \Z^K_0 \}.
\]
Total space is now $ X= \FJ \times \XK \times \Xinfty$
with projections $\pi_\kappa$, $\pi_K$ and $\pi_\infty$.
Whenever convenient we identify the finite dimensional subspaces of $X$ or $\X_0$ with finite dimensional spaces.
\begin{remark}\label{r:matrixmatrix}
For linear operations $M$ on $\FJ \times \XK$ we will use the notation
\begin{alignat*}{1}
  \pi_\kappa M &= M_{11} \pi_\kappa + M_{12} \pi_K ,\\
  \pi_K M &= M_{21} \pi_\kappa + M_{22} \pi_K,
\end{alignat*}
hence in matrix notation
\[
   M = \left( \begin{array}{cc} M_{11} & M_{12} \\ M_{21} & M_{22} \end{array} \right),
\]
with $M_{11}$ a $J\times J$ matrix, $M_{12}$ a $J \times N$ matrix, $M_{21}$ an $N \times J$ matrix, and $M_{22}$ an $N \times N$ matrix.
\end{remark}

We compute numerically an approximate zero $\bx=(\bkappa,\bb) \in \RJ_+ \times \X_0^K$
of 
\[
  (\pi_\kappa+\pi_K) \FF(x) =0.
\]
\begin{remark}
We will restrict attention to $(\bkappa,\bb) \in \Ssym$, replacing $\bb$ by $\frac{1}{2}(\bb+\gammaconj \bb)$ if needed. Since $\bkappa$  naturally lies in $\R^J_+$, in fact we restrict attention to 
\[
  \Ssym_+ \bydef  \Ssym \cap (\FJ_+ \times \X_0)  = 
  \{ x=(\kappa,b) \in \Ssym : \kappa \in \RJ+ \}.
\]
\end{remark}
We then compute numerically the Jacobian 
\[
  M = D \bigl[(\pi_\kappa+\pi_K) \, \FF \circ (\pi_\kappa+\pi_K)\bigr] (\bx)
\]
of the finitely truncated problem, evaluated at the numerical zero.
Finally, we invert the matrix~$M$ numerically to obtain a matrix~$A$,
which may be decomposed into blocks as introduced above. We use this matrix~$A$ to set up the fixed point problem.
The tail part of the full Jacobian of $\FF$ will be approximated by
\begin{equation}\label{e:defLambda}
  (\Lambda b)_k \bydef \PP(\Dk \bkappa) b_k 
  \qquad\text{for all } k \in \ZY_0.
\end{equation}
In order to invert this on $\X^\infty_0$, we assume that $K$ is sufficiently large, so that $\PP(\Dk \bkappa)$ has fixed sign. In particular we choose 
\begin{equation}\label{e:KyP}
  K > \yP^2,
\end{equation}
so that, in view of the choice~\eqref{e:knorm} for the norm $\knorm$,
we have $\PP(\Dk \bkappa)>0$ for $\knorm > K$.
We then set
\begin{equation*}
  (\Lambda^{-1} b)_k \bydef
  \begin{cases} 
	     0 & \quad\text{for  } \knorm \leq K , \\
		 \frac{1}{\PP(\Dk \bkappa)} b_k
   & \quad\text{for  }  \knorm > K .
   \end{cases}
\end{equation*}
The diagonal operators $\Lambda$ and $\Lambda^{-1}$ are inverses on $\X^\infty_0$.

With these preliminaries in place, and writing $x=(\kappa,b)$, we study the   (fixed point) operator 
\begin{equation}\label{e:defT}
  T(x) \bydef  x - \AA \FF(x)
\end{equation}
 with the linear operator $\AA$ defined through
\begin{equation}\label{e:defAA}
  (\pi_\kappa + \pi_K)  \AA x =  A (\pi_\kappa + \pi_K)  x
  \qquad
  \pi_\infty \AA x = \Lambda^{-1} \pi_\infty x .
\end{equation}

We work on a product neighbourhood (ball) of the form
\[
  \BB_{(r_1,r_2)}(x) = \{ (\kappa,b) : 
  |\kappa-\pi_\kappa x|_{\FJ} \leq r_1 , \|b - \pi_b x\|_{\sym} \leq  r_2 \}.
\]
where we write $r=(r_1,r_2)$.
We will also use the conjugate symmetric subset of the ball
\[
  \BBsym_{r}(x) \bydef \BB_r(x) \cap \Ssym = \{ \tilde{x} \in \BB_r(x)  : \gammaconj x = x \}.
\]
In Section~\ref{s:estimates} we will establish estimates of the form
\begin{subequations}\label{e:tenbounds}
\begin{alignat}{2}
  | \pi_\kappa [T (\bx) -\bx] |_{\FJ} &\leq \YY{1} \\  
  \| \pi_b [T (\bx) -\bx] \|_{\X_0} &\leq \YY{2} \\
  \|  \pi_\kappa D_\kappa T (\bx)  \|_{B(\FJ,\FJ)}  &\leq \ZY{1}_1  \label{e:boundZ11}\\
  \|  \pi_\kappa D_b T (\bx)  \|_{B(\X_0,\FJ)}  &\leq \ZY{1}_2  \\
  \|  \pi_b D_\kappa T (\bx)  \|_{B(\FJ,\X_0)}  &\leq \ZY{2}_1  \\
  \|  \pi_b D_b T (\bx)  \|_{B(\X_0,\X_0)}  &\leq \ZY{2}_2   \\
  \| \pi_\kappa [D_\kappa T (x)  - D_\kappa T (\bx)] \|_{B(\FJ,\FJ)}  &\leq \WY{1}_{11}r_1 + \WY{1}_{12}r_2  &\qquad& 
  \text{for all } x \in \BB_r(\bx)   \label{e:boundW11} \\
  \|  \pi_\kappa [D_b T (x) -D_b T(\bx)]  \|_{B(\X_0,\FJ)}  &\leq \WY{1}_{21}r_1 + \WY{1}_{22}r_2   &\qquad&
  \text{for all } x \in \BBsym_r(\bx) \\
  \| \pi_b [D_\kappa T (x)  - D_\kappa T (\bx)] \|_{B(\FJ,\X_0)}  &\leq \WY{2}_{11}r_1 + \WY{2}_{12}r_2  &\qquad&
  \text{for all } x \in \BBsym_r(\bx) \\
  \| \pi_b [D_b T (x) - D_b T(\bx)]  \|_{B(\X_0,\X_0)}  &\leq 
  \WY{2}_{21}r_1 + \WY{2}_{22}r_2   &\qquad&
  \text{for all } x \in \BBsym_r(\bx)  \label{e:boundW22}. 
\end{alignat}
We recall that we assume the center $\bx$ of the ball to be in $\Ssym$,
so that $\BBsym_r(\bx)$ is nonempty.
These estimates will be valid for $0 \leq r_1 \leq \rstar_1$
and $0 \leq r_1 \leq \rstar_2$, for some choice of $\rstar = (\rstar_1,\rstar_2) \in \R^2_+$.
\end{subequations}\

In the following we will often write 
\[ 
 \WY{i}_{i'}(r) \bydef \WY{i}_{i'1}r_1+\WY{i}_{i'2}r_2 \qquad\text{for } i,i'=1,2.
\]
We define the radii polynomials 
\begin{subequations}\label{e:radpols12}
\begin{alignat}{1}
   p_1(r) &\bydef \YY{1} + r_1 [\ZY{1}_1 + \tfrac{1}{2} \WY{1}_1(r) - 1] + r_2 [\ZY{1}_2 + \tfrac{1}{2}\WY{1}_2(r) ] ,\\
   p_2(r) &\bydef \YY{2} + r_1 [\ZY{2}_1 + \tfrac{1}{2}\WY{2}_1(r)] + r_2 [\ZY{2}_2 + \tfrac{1}{2}\WY{2}_2(r) - 1] . 
\end{alignat}
\end{subequations}
Since the dependence of $\W_{ii'}$ is polynomial, we call these \emph{radii polynomials}.
As we will see in the proof of Theorem~\ref{thm:contraction}, the operator $T$ maps $\BB_r$ into itself when $p_1(r)$ and $p_2(r)$ are both negative. 
Contractivity of $T$ on $\BB_r$ is controled by the $2\times 2$ matrix
\begin{equation}\label{e:defM}
  \M(r) \bydef \left[ 
   \begin{array}{cc}
	   \ZY{1}_1 + \WY{1}_1(r)  & \ZY{1}_2 + \WY{1}_2(r)  \\[1mm]
	   \ZY{2}_1 + \WY{2}_1(r)  & \ZY{2}_2 + \WY{2}_2(r)  
   \end{array}
   \right] .
\end{equation}
It will become apparent in the proof of Theorem~\ref{thm:contraction} that we need the dominant (Perron-Frobenius) eigenvalue 
of this positive matrix to be less than $1$.
We express this eigenvalue in terms of the trace and determinant of $\M(r)$:
\[
  \sigma(r) \bydef \frac{\tr \M(r) + \sqrt{(\tr \M(r))^2 - 4 \det \M(r) }}{2}.
\]
The demand $\sigma(r)<1$ is equivalent to
requiring that the polynomials
\begin{subequations}\label{e:radpols34}
\begin{alignat}{1}
   \tp_3(r) &\bydef \tr \M(r) -2 ,\\
   \tp_4(r) &\bydef \tr \M(r) - \det M(r)  - 1 ,
\end{alignat}
\end{subequations}
are negative.
Hence we aim to find $0<\hr \leq \rstar$, with inequalities interpreted component-wise, such that 
\begin{subequations}
\label{e:pleq0}
\begin{alignat}{2}
  p_1(\hr_1, \hr_2) &<0, \qquad& 
  p_2(\hr_1, \hr_2) &<0, \label{e:p12ll0}\\
  \tp_3(\hr_1, \hr_2) &<0, \qquad&
  \tp_4(\hr_1, \hr_2) &<0. \label{e:tp34ll0}
\end{alignat}
\end{subequations}

\begin{remark}\label{r:minimax}
For positive $2 \times 2$ matrices $\M$ one may reduce the demand that the dominant eigenvalue is less than $1$ in terms of the trace and the determinant. 
More generally, consider a positive $m \times m$ matrix $\M$.
The Collatz-Wielandt formula provides the minimax characterization
\begin{equation}\label{e:minimax}
  \sigma = \min_{y \in \R^m_+} \max_{1\leq i \leq m} \frac{(\M y)_i}{y_i}
\end{equation}
for the dominant eigenvalue.
In particular, when the dimension of the matrix is larger it is not difficult to obtain rigorous upper bounds on $\sigma(r)$ by choosing appropriate test vectors $y\in \R^m_+$.
\end{remark}

\begin{theorem}\label{thm:contraction}
Assume $\bx \in \Ssym_+$. Assume the matrix $A$ is invertible and $\gammaconj A = A \gammaconj$. 
Let $\rstar \in \R^2_+$ with $\rstar_1 < 1$.
Let $\YY{i} , \ZY{i}_{i'}, \WY{i}_{i'i''} \in \R_+$ satisfy the bounds~\eqref{e:tenbounds} for $i,i',i''=1,2$ and $0 \leq r \leq \rstar$. 
Let $p_1$, $p_2$ and $\tp_3$, $\tp_4$ be as defined in~\eqref{e:radpols12}
and ~\eqref{e:radpols34}, respectively.
If $\hr_1,\hr_2 >0$ 
are such that $\hr \leq \rstar$
and  inequalities~\eqref{e:pleq0} are satisfied, 
then
\begin{thmlist}
\item
$\FF$ has a unique zero $\hx=(\hkappa,\hb)$ in $\BBsym_{\hr}(\bx)$; 
\item 
$\hb$ corresponds to a $\G$-invariant real-valued periodic solution 
\[
  \hu(\x) = \sum_{k \in \Z^3} (\sigma(m\e_0+\hb))_k \exp(\textup{i} \L_{\hkappa} k \cdot \x)
\]
of the PDE~\eqref{e:PDEOK}; 
\item 
the domain of periodicity $\Omega_{\hkappa}$, given by~\eqref{e:omegakappa}, is
such that the energy is stationary with respect to variations in its
($\G$-symmetry respecting) proportions. 
\end{thmlist}
\end{theorem}
\begin{proof}
We observe that $T$ preserves conjugate symmetry, i.e., it maps $\Ssym$ to itself. Indeed, it follows from Remark~\ref{r:extendconj} combined with Equations~\eqref{e:hfconjequivariant} and~\eqref{e:defFF} that  $\FF(\gammaconj x) = \gammaconj \FF(x)$ for any $x \in \FJ_+ \times \X_0$.
Since $A \gammaconj = \gammaconj A$ by assumption, we conclude from~\eqref{e:defAA} that $\AA\gammaconj=\gammaconj\AA$.
This implies that $T(\gammaconj x) = \gammaconj T(x)$, hence $T$ restricts to map from $\Ssym_+$ to $\Ssym$.

Next we show that $T$ maps $\BBsym_{\hr}(\bx)$ to itself.
Fix any $x = (\kappa,b) \in \Ssym$ such that $|\kappa- \bkappa |_{\FJ} \leq \hr_1$ and $\|b- \bb \|_{\X_0} \leq \hr_1$.
Then 
\[
  |\pi_\kappa T(x) - \bkappa |_{\FJ}
  \leq
    |\pi_\kappa [T(x) - T(\bx)]  |_{\FJ}  + | \pi_\kappa[T(\bx) - \bx] |_{\FJ}
	\leq |\pi_\kappa [T(x) - T(\bx)]  |_{\FJ} +    \YY{1}.
\]
We estimate
\begin{alignat*}{1}
 |\pi_\kappa [T(x) - T(\bx)] |_{\FJ} &= \left|
 \int_0^1 \left\{ \pi_\kappa D_\kappa T((1-s)x+s\bx) (\kappa-\bkappa)  + 
 \pi_\kappa D_b T((1-s)x+s\bx) (b-\bb) \right\} ds 
  \right|_{\FJ} \\ 
 & \leq |\kappa-\bkappa|_{\FJ}  \int_0^1 \| \pi_\kappa D_\kappa T((1-s)x+s\bx) \|_{B(\FJ,\FJ)} ds   \\
 & \hspace*{1cm} +
 \| b-\bb\|_{\X_0}
 \int_0^1 \| \pi_\kappa D_b T((1-s)x+s\bx) \|_{B(\X_0,\FJ)} ds \, .
\end{alignat*}
Since $\Ssym$ is convex and $\WY{1}_1 (r)$ is linear in $r$,  we obtain
from~\eqref{e:boundZ11} and~\eqref{e:boundW11}
\begin{alignat*}{1}
\| \pi_\kappa D_\kappa T((1-s)x+s\bx) \|_{B(\FJ,\FJ)} 
& = \| \pi_\kappa D_\kappa T(\bx) + D_\kappa   T(\bx+s(x-\bx)) - D_\kappa T(\bx) \|_{B(\FJ,\FJ)} \\
& \leq \| \pi_\kappa D_\kappa T(\bx) \|_{B(\FJ,\FJ)}  +  \|D_\kappa   T(\bx+s(x-\bx)) - D_\kappa T(\bx) \|_{B(\FJ,\FJ)} \\
& \leq \ZY{1}_1 +  \WY{1}_1(s\hr_1,s\hr_2)
= \ZY{1}_1 +  s\WY{1}_1(\hr_1,\hr_2).
\end{alignat*}
Similarly, we bound
\[
\| \pi_\kappa D_b T((1-s)x+s\bx) \|_{B(\X_0,\FJ)} \leq 
 \ZY{1}_2 + s \WY{1}_2(\hr_1,\hr_2). 
\]
We combine the above estimates into
\[
 |\pi_\kappa T(x) - \bkappa |_{\FJ} \leq
  \YY{1} + \hr_1 \int_0^1 \ZY{1}_1 + s \WY{1}_1(\hr)  ds +  
  \hr_2  \int_0^1 \ZY{1}_2 + s \WY{1}_2(\hr)  ds 
  = p_1(\hr) + \hr_1  < \hr_1.
\]
An entirely analogous argument leads to the estimate
\[
 \|\pi_b T(x) - \bb \|_{\X_0} \leq 
  = p_2(\hr) + \hr_2  < \hr_2.
\]
We conclude that $T$ maps $\BBsym_{\hr}(\bx)$ to itself.

Next we want to establish that $T$ is contractive on $\BBsym_{\hr}(\bx)$,
hence we need to choose a norm on $\FJ \times \X_0$.
Consider the dominant eigenvalue $\sigma(\hr)$ of $\M(\hr)$,
and let $\rho=[\rho_1,\rho_2]^T \in \R^2_+$ be an associated eigenvector.
The we choosing as the norms on the product space $\FJ \times \X_0$
\[
  \| (\kappa , b) \|_{\rho} =   \max \left\{ \frac{|\kappa|_{\FFJ}}{\rho_1}, \frac{\| b \|_{\X_0}}{\rho_2}   \right\} .
\]
We denote $\FJ \times \X_0$ interpreted as a Banach space with norm $\|x\|_\rho$ by $X_\rho$. 
We fix $x\in \BBsym_{\hr}(\bx)$ and write
With this norm we can interpret the linear operator
$DT \in B(X_\rho,X_\rho)$ in terms of a $2 \times 2$ block structure as in Remark~\ref{r:matrixmatrix}, with corresponding matrix~\eqref{e:defM}.
with a weighted $\infty$-norm. 
Indeed, the minimax characterization~\eqref{e:minimax} is the motivation for choosing the norm $\|x\|_\rho$ on the product space.
Hence we obtain 
\begin{alignat*}{1}
   \| DT(x) \|_{B(X_\rho,X_\rho)} & =    
   \max\left\{ 
   \frac{\rho_1 \| \pi_\kappa D_\kappa T(x)\|_{B(\FJ,\FJ)} +
   \rho_2 \| \pi_\kappa  D_\kappa T (x)\|_{B(\X_0,\FJ)} }{\rho_1} , \right.\\
   & \hspace*{4cm} \left.
   \frac{\rho_1 \| \pi_b D_\kappa T(x)\|_{B(\FJ,\X_0)} +
    \rho_2 \| \pi_b D_\kappa T(x) \|_{B(\X_0,\X_0)} }{\rho_2}
    \right\} .
\end{alignat*}
By using the triangle inequality and~\eqref{e:boundZ11}--\eqref{e:boundW22}, 
we then obtain
\begin{alignat*}{1}
   \| DT (x)\|_{B(X_\rho,X_\rho)} &    
   \leq 
   \max\left\{ 
   \frac{\rho_1 (\ZY{1}_1+\WY{1}_1 (\hr)) +
   \rho_2 (\ZY{1}_2+\WY{1}_2 (\hr))}{\rho_1} , 
   \right.\\ & \hspace*{4cm} \left.
   \frac{\rho_1 (\ZY{2}_1+\WY{2}_1 (\hr)) +
    \rho_2 (\ZY{2}_2+\WY{2}_2 (\hr)) }{\rho_2}
    \right\} .
   \\
   & = \sigma(\hr) <1.
\end{alignat*}
Since the estimate is uniform for $x \in \BBsym_{\hr}(\bx)$
we conclude that $T$ is contractive on $\BBsym_{\hr}(\bx)$
for the norm $\|x\|_\rho$.

From the above and the Banach contraction mapping theorem 
we conclude that $T$ has a unqiue fixed point $\hx$ in $\BBsym_{\hr}(\bx)$.
Since the matrix $A$ is invertible by assumptoin, it follows from~\eqref{e:defAA} that $\AA$ is invertible, hence injective.
We conclude that 
$\hx$ is the unique zero of $\FF$ in $\BBsym_{\hr}(\bx)$. This finishes the proof of part (a).

Part (b) follows from Theorem~\ref{thm:solvePDE}. We note that it follows from part (a) that $\hkappa$ is real-valued, whereas the assumption that $\hr_1 \leq \rstar_1<1$ implies that $\hkappa_j>0$ for all $1\leq j \leq J$.

Part (c) follows from $H_j(\hkappa,\hb)=h_j(\hkappa,\sigma(m\e_0+\hb))=0$ 
and Equation~\eqref{e:dEdkappa}.
\end{proof}

\begin{remark}
Theorem~\ref{thm:contraction} is a variation on a general strategy. Some of the notation was introduced in~\cite{yamamoto}, while the idea to collect the necesary inequalities in radii polynomials stems from~\cite{DLM}. We do not review the relevant literature here, but refer instead to~\cite{ariolikochintegration,plumbridge,JBJPAMS} and then references therein.
There are some ingredients to the theorem that are less standard. First, we restrict attention to the conjugate symmetric set, which simplifies the estimates. Second, following~\cite{JBintro} (see also \cite{JBJonathan}) we do not choose a norm on the product space $\FJ \times \X_0$ a priori. Indeed, we keep track of the different components of the derivatives when performing the estimates. This refinement leads to the two polynomials $p_1(r_1,r_2)$ and $p_2(r_1,r_2)$ depending on two variables rather than a single polynomial in a single variable. Moreover, it allows us to separate the invariance of $\BB_{\hr}(\bx)$ from contractivity. The norm chosen for contractivity has been optimized (in the sense explained in Remark~\ref{e:minimax}), which improves on the arguments in~\cite{JBintro}. We refer to~\cite{JBJFbif} for a similar argument in the context of continuation. Finally, as in~\cite{NS} the splitting of the Jacobian into a $Z$-part and a $W$-part leads to a factor $\frac{1}{2}$ in the $W$-terms in $p_1$ and $p_2$.
\end{remark}

\begin{remark}
One may simplify the conditions~\eqref{e:pleq0} to the \emph{stronger} requirements
\begin{alignat*}{1}
\YY{1} + \hr_1 [\ZY{1}_1 + \WY{1}_1(\hr) - 1] + r_2 [\ZY{12} + \WY{1}_2(\hr) & < 0 \\
\YY{2} + \hr_1 [\ZY{2}_1 + \WY{2}_1(\hr)] + r_2 [\ZY{22} +\WY{2}_2(\hr) - 1] & < 0. 
\end{alignat*}	
Indeed, when these inequalities are satisfied the estimate $\sigma(\M(\hr))<1$ on the dominant eigenvalue is obtained by using the test vector $y=(\hr_1,\hr_2)^T$
in~\eqref{e:minimax}. This corresponds to the approach taken in~\cite{JBintro}.
\end{remark}

\begin{remark}
The domains $\Omega_i \bydef \{ r \in \R^2_+ : p_i(r)<0 \}$ are convex for $i=1,2$. 
Furthermore, if $(r_1,r_2) \in \Omega_1$, then $(r_1,r) \in \Omega_1$ for all $0 < r < r_2$, and similarly for $\Omega_2$ (with the roles of $r_1$ and $r_2$ exchanged).
We conclude that if $r^{[1]}, r^{[2]} \in \Omega_1 \cap \Omega_2$, which we assume to be nonempty, then so is
$(\min\{r^{[1]}_1,r^{[2]}_1\},\min\{r^{[1]}_2,r^{[2]}_2\})$. 
It follows that there is a \emph{minimal radius vector} $r_{\min} \in
\overline{\Omega_1 \cap \Omega_2}$, i.e., the point in the latter set which is closest to the origin. In turn this implies that there exists a
direction $\hat{y} \in \R^2_+$ such that $\nabla p_i(r_{\min}) \cdot \hat{y} <0$
for $i=1,2$.

Now assume that $\WY{1}_{12}=\WY{1}_{21}$ and $\WY{2}_{12}=\WY{2}_{21}$, which
is natural when the corresponding estimates are derived by bounding the second
derivatives $\pi_\kappa D_b D_\kappa T(x)$ and $\pi_b D_b D_\kappa T(x)$,
respectively. Then the estimate $\sigma(\M(\hr))<1$ is obtained by using the
test vector $y=\hat{y}$. Hence under the symmetry condition
$\WY{i}_{12}=\WY{i}_{21}$ the inequalities~\eqref{e:tp34ll0} are implied
by~\eqref{e:p12ll0}. 
%\red{NEED TO CHECK THAT THIS IS TRUE!}
\end{remark}

\begin{remark} In practice we verify the assumptions on $A$ in
Theorem~\ref{thm:contraction} as follows.
After computing a numerical inverse $A$ of the
approximate Jacobian $M$ we replace it by 
$\frac{1}{2} (A+ \gammaconj A \gammaconj)$ 
to ensure that it preserves conjugation symmetry. For this new matriox $A$ we
then compute the matrix $1$-norm of $I-AQ$. When
$\| I-AQ \|_1 <1$ we conclude that the matrix $A$ is invertible.
Finally we note that $\gammaconj A \gammaconj$ is represented by the matrix 
$\Gamma_0  \overline{A} \, \overline{\Gamma_0}$, where the overline denotes elementwise complex conjugate and, with the block structure as in Remark~\ref{r:matrixmatrix},
\[
  \Gamma_0 = 
  \left( \begin{array}{cc} \delta_{jj'} & 0 \\
  0 & \phi_{k} \delta_{k\tau(k)} 
  \end{array} \right),
\]
with $\phi$ and $\tau$ introduced in Remark~\ref{r:explicitGamma}.
\end{remark}

\begin{remark}\label{r:errorcontrol}
Let 
\[
  \bu(\x) \bydef \sum_{k \in \Z^3,\knorm\leq K} (\sigma(m\e_0+\bb))_k \exp(\textup{i} \L_{\bkappa} k \cdot \x)
\]
be the approximate periodic solution.
Then we have the following error control:
\[
	\bigl\|\hu (\x) - \bu\bigl( (\L_{\bkappa}^T)^{-1}  \L_{\hkappa}^T  \x\bigr) \bigr\|_\infty \leq \hr_2 ,
\]
where the rescaling is necessary to correct for dephasing. 
Moreover, $|\hkappa_j - \bkappa_j| \leq \bkappa_j \hr_1 $
for  $1\leq j \leq J$.
\end{remark}

\begin{remark}
In addition to~\eqref{e:KyP}, in Section~\ref{s:estimates}, where to derive explicit bounds, we will put additional restrictions on the computational parameter $K$, namely
\begin{equation}\label{e:Krestrictions}
  K^2 > \max\{ y_P , \gamma (1-r_1^*)^{-1} , 2  \}.
\end{equation}
\end{remark}

The operator norms appearing in~\eqref{e:tenbounds}
are given explicitly by
\begin{alignat}{1}
  \|Q\|_{B(\FJ,\FJ)} &= 
  \max_{1\leq j \leq J} \bkappa_j^{-1} \sum_{j=1}^J | Q_{j j'}| \bkappa_{j'} \,,
  \label{e:norm11}\\	
  \|Q\|_{B(\X_0,\FJ)} &= 
  \sup_{k\in\ZY_0} \omega_{k}^{-1} \max_{1\leq j \leq J} \bkappa_j^{-1} |Q_{jk}| \,,
  \label{e:norm12} \\	
  \|Q\|_{B(\FJ,\X_0)} &=  
  \max_{\epsilon_j= \pm 1 } \sum_{k\in\ZY_0} \omega_k
  	 	\biggl| \sum_{j=1}^J \epsilon_j \bkappa_j Q_{k j} \biggr| \,,
  \label{e:norm21}\\	
  \|Q\|_{B(\X_0,\X_0)} &= 
  \sup_{k\in\ZY_0} \omega_{k}^{-1} \sum_{k'\in\ZY_0} \omega_k |Q_{k'k}| \,.
  \label{e:norm22}	
\end{alignat}
When the operators reduce to finite matrices (e.g.~$A_{ii'}$, $i,i'=1,2$)
then the suprema reduce to maxima and the infinite sums reduce to finite ones,  hence in that case these expressions can be evaluated explicitly.

For future use we note that, for both $X'=\FJ$ and $Y=\X_0$,
\begin{alignat}{1}
\| Q \|_{B(\X_0,X')} &= 
\sup_{k\in\ZY_0} \omega_k^{-1} \| Q \e_k\|_{X'} \label{e:l1sup} \\ 
 &= \max\bigl\{ \| Q \pi_N \|_{B(\X_0,X')}, \| Q(I-\pi_N)\|_{B(\X_0,X')} \bigr\}
\qquad \text{for any } N>0.  \label{e:splitl1norm}
\end{alignat}



